Distillation Improves Visual Place Recognition for Low Quality Images

Real-time visual localization often utilizes online computing, for which query images or videos are transmitted to remote servers for visual place recognition (VPR). However, limited network bandwidth necessitates image-quality reduction and thus the degradation of global image descriptors, reducing VPR accuracy. We address this issue at the descriptor extraction level with a knowledge-distillation methodology that learns feature representations from high-quality images to extract more discriminative descriptors from low-quality images. Our approach includes the Inter-channel Correlation Knowledge Distillation (ICKD) loss, Mean Squared Error (MSE) loss, and Triplet loss. We validate the proposed losses on multiple VPR methods and datasets subjected to JPEG compression, resolution reduction, and video quantization. We obtain significant improvements in VPR recall rates under all three tested modalities of lowered image quality. Furthermore, we fill a gap in VPR literature on video-based data and its influence on VPR performance. This work contributes to more reliable place recognition in resource-constrained environments.

==> Table_Figure_Wrappers/table2_initial.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[t]
  \centering
    \begin{tabular}{cr|rrrr|rrrr|rrrr}
    \toprule
    \multirow{2}[2]{*}{VPR Methods} & \multicolumn{1}{c|}{\multirow{2}[2]{*}{Configuration}} & \multicolumn{4}{c|}{Mapillary SLS} & \multicolumn{4}{c|}{Nordland} & \multicolumn{4}{c}{Tokyo 24/7} \\
          &       & \multicolumn{1}{l}{R@1} & \multicolumn{1}{l}{R@2} & \multicolumn{1}{l}{R@5} & \multicolumn{1}{l|}{R@10} & \multicolumn{1}{l}{R@1} & \multicolumn{1}{l}{R@2} & \multicolumn{1}{l}{R@5} & \multicolumn{1}{l|}{R@10} & \multicolumn{1}{l}{R@1} & \multicolumn{1}{l}{R@2} & \multicolumn{1}{l}{R@5} & \multicolumn{1}{l}{R@10} \\
    \midrule
    \multirow{4}[2]{*}{MixVPR} & pretrained (raw) & \textcolor{gray}{82.73} & \textcolor{gray}{86.67} & \textcolor{gray}{89.73} & \textcolor{gray}{91.65} & \textcolor{gray}{57.79} & \textcolor{gray}{64.13} & \textcolor{gray}{71.49} & \textcolor{gray}{76.41} & \textcolor{gray}{87.30} & \textcolor{gray}{89.52} & \textcolor{gray}{92.06} & \textcolor{gray}{93.65} \\
          & pretrained (90\%) & 71.87 & 76.61 & 81.22 & 84.19 & 31.05 & 36.12 & 44.13 & 51.23 & 66.03 & 73.33 & 78.73 & 82.22 \\
          & finetuned (90\%) & \textcolor{green}{5.8\%} & \textcolor{green}{5.1\%} & \textcolor{green}{4.4\%} & \textcolor{green}{3.6\%} & 43.1\% & 39.6\% & 33.2\% & 28.2\% & \textcolor{green}{14.5\%} & \textcolor{green}{10.4\%} & 7.6\% & 6.6\% \\
          & ICKD (90\%) & 6.0\% & 4.8\% & 4.0\% & 3.5\% & \textcolor{green}{48.3\%} & \textcolor{green}{45.9\%} & \textcolor{green}{38.0\%} & \textcolor{green}{31.2\%} & 12.5\% & 8.2\% & \textcolor{green}{8.1\%} & \textcolor{green}{8.1\%} \\
    \midrule



    \multirow{4}[2]{*}{CricaVPR} & pretrained (raw) & \textcolor{gray}{74.74} & \textcolor{gray}{80.92} & \textcolor{gray}{86.09} & \textcolor{gray}{88.75} & \textcolor{gray}{87.64} & \textcolor{gray}{90.65} & \textcolor{gray}{94.24} & \textcolor{gray}{95.80} & \textcolor{gray}{90.16} & \textcolor{gray}{92.38} & \textcolor{gray}{95.56} & \textcolor{gray}{96.19} \\
          & pretrained (90\%) & 68.14 & 74.41 & 80.24 & 83.19 & 63.51 & 69.71 & 77.46 & 82.64 & 74.29 & 79.68 & 84.76 & 87.94 \\
          & finetuned (90\%) & 0.0\% & 0.0\% & 0.0\% & 0.0\% & \textcolor{red}{-4.7\%} & \textcolor{red}{-4.2\%} & \textcolor{red}{-3.8\%} & \textcolor{red}{-3.4\%} & 6.8\% & 5.6\% & 2.9\% & 2.2\% \\
          & ICKD (90\%) & \textcolor{green}{1.3\%} & \textcolor{green}{1.9\%} & \textcolor{green}{1.4\%} & \textcolor{green}{1.4\%} & \textcolor{green}{18.3\%} & \textcolor{green}{15.5\%} & \textcolor{green}{11.5\%} & \textcolor{green}{8.5\%} & \textcolor{green}{9.4\%} & \textcolor{green}{6.4\%} & \textcolor{green}{7.1\%} & \textcolor{green}{5.4\%} \\

    \midrule
    
    \multirow{4}[2]{*}{\makecell{DINOv2 \\ SALAD}} & pretrained (raw) & \textcolor{gray}{89.20} & \textcolor{gray}{92.40} & \textcolor{gray}{94.70} & \textcolor{gray}{95.84} & \textcolor{gray}{88.08} & \textcolor{gray}{90.94} & \textcolor{gray}{94.13} & \textcolor{gray}{95.98} & \textcolor{gray}{97.14} & \textcolor{gray}{97.46} & \textcolor{gray}{98.73} & \textcolor{gray}{99.05} \\
          & pretrained (90\%) & 84.60 & 88.85 & 91.89 & 93.68 & 67.90 & 73.88 & 80.40 & 84.24 & 89.21 & 92.06 & 95.87 & 96.51 \\
          & finetuned (90\%) & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & \textcolor{red}{-0.5\%} & \textcolor{red}{-0.9\%} & 0.0\% & \textcolor{red}{-0.7\%} & 0.0\% & \textcolor{red}{-1.0\%} & 0.0\% \\
          & ICKD (90\%) & \textcolor{green}{0.6\%} & \textcolor{green}{0.5\%} & \textcolor{green}{0.2\%} & \textcolor{green}{0.3\%} & \textcolor{green}{2.3\%} & \textcolor{green}{2.5\%} & \textcolor{green}{1.4\%} & \textcolor{green}{1.4\%} & \textcolor{green}{1.8\%} & \textcolor{green}{1.4\%} & \textcolor{green}{0.3\%} & \textcolor{green}{0.0\%} \\

    \midrule
    

    \multirow{4}[2]{*}{NetVLAD} & pretrained (raw) & \textcolor{gray}{49.29} & \textcolor{gray}{55.24} & \textcolor{gray}{62.07} & \textcolor{gray}{67.29} & \textcolor{gray}{5.51} & \textcolor{gray}{6.67} & \textcolor{gray}{8.62} & \textcolor{gray}{11.38} & \textcolor{gray}{60.63} & \textcolor{gray}{63.81} & \textcolor{gray}{69.21} & \textcolor{gray}{74.29} \\
          & pretrained (90\%) & 32.60 & 37.67 & 44.92 & 50.13 & 1.99  & 3.01  & 4.93 & 7.07 & 27.94 & 33.02 & 41.90 & 47.94 \\
          & finetuned (90\%) & 0.1\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% & 0.0\% \\
          & MSE (90\%) & \textcolor{green}{13.6\%} & \textcolor{green}{14.1\%} & \textcolor{green}{11.4\%} & \textcolor{green}{10.0\%} & \textcolor{green}{27.6\%} & \textcolor{green}{14.3\%} & \textcolor{red}{-3.6\%} & \textcolor{red}{-10.3\%} & \textcolor{green}{29.5\%} & \textcolor{green}{19.2\%} & \textcolor{green}{14.4\%} & \textcolor{green}{10.6\%} \\

    \midrule

    \multirow{3}[2]{*}{AnyLoc} & pretrained (raw) & \textcolor{gray}{56.51} & \textcolor{gray}{62.31} & \textcolor{gray}{68.28} & \textcolor{gray}{72.89} & \textcolor{gray}{12.90} & \textcolor{gray}{16.23} & \textcolor{gray}{20.18} & \textcolor{gray}{24.28} & \textcolor{gray}{88.25} & \textcolor{gray}{91.11} & \textcolor{gray}{94.92} & \textcolor{gray}{96.83} \\
          & pretrained (90\%) & 48.04 & 56.45 & 63.84 & 69.17 & 10.11 & 12.97 & 17.86 & 21.92 & 83.49 & 87.30 & 91.75 & 95.87 \\
          & \makecell{ICKD + \\ Triplet (90\%)} & \textcolor{green}{2.1\%} & \textcolor{green}{2.7\%} & \textcolor{green}{4.2\%} & \textcolor{green}{3.5\%} & \textcolor{green}{17.2\%} & \textcolor{green}{14.6\%} & \textcolor{green}{8.5\%} & \textcolor{green}{11.6\%} & \textcolor{red}{-6.8\%} & \textcolor{red}{-1.8\%} & \textcolor{green}{1.7\%} & \textcolor{red}{-1.0\%} \\

    \bottomrule
    \end{tabular}%
\caption{Performance comparison of various Visual Place Recognition (VPR) methods across three benchmark datasets: Mapillary SLS, Nordland, and Tokyo 24/7. The table presents recall rates (R@1, R@2, R@5, R@10) for different configurations, including \textit{pretrained}, \textit{finetuned}, and \textit{ICKD + Triplet} models. For each method, the third and fourth rows (finetuned 90\% and ICKD 90\%) show the percentage improvements or declines over the \textit{pretrained (90\%)} configuration. \textcolor{green}{Green} indicates improvements, and \textcolor{red}{red} highlights any negative changes. Distillation using ICKD and Triplet loss demonstrates significant gains, particularly on the Nordland and Tokyo 24/7 datasets, underscoring the potential of distillation to enhance VPR performance.}


  \label{table:mainres}%
\end{table*}%
